On the Coherence of Large-Scale Networks with Distributed PI and PD Control

We consider distributed control of double-integrator networks, where agents are subject to stochastic disturbances. We study performance of such networks in terms of coherence, defined through an H2 norm metric that represents the variance of nodal state fluctuations. Specifically, we address known performance limitations of the standard consensus protocol, which cause this variance to scale unboundedly with network size for a large class of networks. We propose distributed proportional integral (PI) and proportional derivative (PD) controllers that relax these limitations and achieve bounded variance, in cases where agents can access an absolute measurement of one of their states. This case applies to, for example, frequency control of power networks and vehicular formation control with limited sensing. We discuss optimal tuning of the controllers with respect to network coherence and demonstrate our results in simulations.

==> Figures/FDPD.tex <==
\begin{tikzpicture}
	\pgfplotsset{every tick label/.append style={font=\scriptsize}}
	\pgfplotsset{every axis title/.append style={font=\small}}
		\pgfplotsset{every axis label/.append style={font=\scriptsize}}
	%	\pgfplotsset{every axis/.append style={    height=2.75cm, width=4.5cm, xmin=0, xmax=20,}   }
	%Plot 1 Theta gamma = 0.1
	\begin{axis}
	[name = theta1,
	xlabel={Vehicle position $x$  },
	ylabel={Time $t$},
 y label style={at={(0.12,0.5)}},    
  x label style={at={(0.5,0.1)}},   
    title style = {at={(0.5,0.9)}},   
		height=3.2cm,
	width=5.5 cm,
		xmin=0,
	xmax=72,
	ymin=0,
	ymax=200,
	ytick={0,100,200},
		title={P control},
	yticklabel style={/pgf/number format/.cd,
		fixed,
		%fixed zerofill,
		precision=4},
	grid=major,
	cycle list name= color list,
	]
	\foreach \x in {1,2,3,4,5,6,7,8,9,10, 11,12,13,14,15,16,17,18,19,20,21,22,23,24,25} {
	\addplot +[mark=none,   ] table[x index=\x,y index=0,col sep=space]{Figures/Plot_data/FDPDsim.txt};
	}	
%		\foreach \x in {1} {
%	\addplot +[mark=none,   ] table[x index=\x,y index=0,col sep=space]{Figures/Plot_data/FDPDsim.txt};
%	}	
	\end{axis}
	

	\begin{axis}
	[at=(theta1.below south west), anchor=above north west,
	yshift=-0.10cm,
	name = theta2,
	xlabel={Vehicle position $x$  },
	ylabel={Time $t$},
 y label style={at={(0.12,0.5)}},    
  x label style={at={(0.5,0.1)}},   
    title style = {at={(0.5,0.9)}},   
			height=3.2cm,
	width=5.5 cm,
	%xmin=0,
	%xmax=20,
		xmin=0,
	xmax=72,
	ymin=0,
	ymax=200,
	ytick={0,100,200},
	yticklabel style={/pgf/number format/.cd,
		fixed,
		%fixed zerofill,
		precision=4},
			title={F-DPD},
	grid=major, cycle list name=color list,
	%height=2.5cm,
	%width=3.5cm,
	]
	\foreach \x in {27,28,29,30,31,32,33,34,35,36,37,38,39,40,41,42,43,44,45,46,47,48,49,50,51} {
	\addplot +[mark=none, ] table[x index=\x,y index=26,col sep=space]{Figures/Plot_data/FDPDsim.txt};
	}	
%		\foreach \x in {27} {
%	\addplot +[mark=none, ] table[x index=\x,y index=26,col sep=space]{Figures/Plot_data/FDPDsim.txt};
%	}
	\end{axis}
			
	
	
	\end{tikzpicture}	

==> Figures/Power.tex <==
\begin{tikzpicture}
		\pgfplotsset{every tick label/.append style={font=\scriptsize}}
	\pgfplotsset{every axis title/.append style={font=\small}}
		\pgfplotsset{every axis label/.append style={font=\scriptsize}}
	%	\pgfplotsset{every axis/.append style={    height=2.75cm, width=4.5cm, xmin=0, xmax=20,}   }
	%Plot 1 Theta gamma = 0.1
	\begin{axis}
	[name = theta1,
	xlabel={Time $t$  },
	ylabel={$\theta$},
 y label style={at={(0.15,0.5)}},    
  x label style={at={(0.5,0.1)}},   
  	title={P control (Droop), $N = 10$},
title style = {at={(0.5,0.9)}},   
		height=3.2cm,
	width=5.5 cm,
		xmin=0,
	xmax=15,
	ymin=-0.5,
	ymax=0.5,
	ytick={-0.5,0,0.5},
	yticklabel style={/pgf/number format/.cd,
		fixed,
		%fixed zerofill,
		precision=4},
	grid=major,
	cycle list name= color list,
	]
	\foreach \x in {1,2,3,4,5,6,7,8,9,10} {
	\addplot +[mark=none,   ] table[x index=0,y index=\x,col sep=space]{Figures/Plot_data/P10.txt};
	}	
%		\foreach \x in {1} {
%	\addplot +[mark=none,   ] table[x index=0,y index=\x,col sep=space]{Figures/Plot_data/P10.txt};
%	}	
	\end{axis}
	

	\begin{axis}
	[at=(theta1.below south west), anchor=above north west,
	name = theta2,
	yshift=-0.1cm,
	name = theta2,
	xlabel={Time $t$  },
	ylabel={$\theta$},
%	ylabel near ticks,
%	xlabel near ticks,
 y label style={at={(0.15,0.5)}},    
  x label style={at={(0.5,0.1)}},   
    title style = {at={(0.5,0.9)}},   
		height=3.2cm,
	width=5.5 cm,
		xmin=0,
	xmax=15,
	ymin=-0.5,
	ymax=0.5,
	ytick={-0.5,0,0.5},
	title={DAPI, $N = 10$},
	yticklabel style={/pgf/number format/.cd,
		fixed,
		%fixed zerofill,
		precision=4},
	grid=major,
	cycle list name= color list,
	]
	\foreach \x in {1,2,3,4,5,6,7,8,9,10} {
	\addplot +[mark=none,   ] table[x index=0,y index=\x,col sep=space]{Figures/Plot_data/DAPI10.txt};
	}	
%		\foreach \x in {1} {
%	\addplot +[mark=none,   ] table[x index=0,y index=\x,col sep=space]{Figures/Plot_data/P10.txt};
%	}	
	
	
	
	\end{axis}
			
		\begin{axis}
	[at=(theta1.right of south east), anchor=left of south west,
	name = omega1,
	xlabel={Time $t$  \textit{(Note scale!)}},
	ylabel={$\theta$ \textit{(Note scale!)}},
 y label style={at={(0.15,0.5)}},    
  x label style={at={(0.5,0.1)}},   
  title style = {at={(0.5,0.9)}},   
			height=3.2cm,
	width=5.5 cm,
	  	title={P control (Droop), $N = 100$},
	%xmin=0,
	%xmax=20,
		xmin=0,
	xmax=80,
	ymin=-0.8,
	ymax=0.8,
	ytick={-0.5,0,0.5},
	yticklabel style={/pgf/number format/.cd,
		fixed,
		%fixed zerofill,
		precision=4},
	grid=major, cycle list name=color list,
	%height=2.5cm,
	%width=3.5cm,
	]
	\foreach \x in {1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20} {
	\addplot +[mark=none,   ] table[x index=0,y index=\x,col sep=space]{Figures/Plot_data/P100.txt};
	}	
%		\foreach \x in {1} {
%	\addplot +[mark=none,   ] table[x index=0,y index=\x,col sep=space]{Figures/Plot_data/P10.txt};
%	}	
	\end{axis}
	

	\begin{axis}
	[at=(omega1.below south west), anchor=above north west,
	yshift=-0.1 cm,
	name = theta2,
	xlabel={Time $t$  },
	ylabel={$\theta$},
 y label style={at={(0.15,0.5)}},    
  x label style={at={(0.5,0.1)}},   
    title style = {at={(0.5,0.9)}},   
  %  ylabel near ticks,
	%xlabel near ticks,
			height=3.2cm,
	width=5.5 cm,
	%xmin=0,
	%xmax=20,
		xmin=0,
	xmax=15,
	ymin=-0.5,
	ymax=0.5,
	ytick={-0.5,0,0.5},
	title={DAPI, $N = 100$},
	yticklabel style={/pgf/number format/.cd,
		fixed,
		%fixed zerofill,
		precision=4},
	grid=major, cycle list name=color list,
	%height=2.5cm,
	%width=3.5cm,
	]
	\foreach \x in {1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20} {
	\addplot +[mark=none,   ] table[x index=0,y index=\x,col sep=space]{Figures/Plot_data/DAPI100.txt};
	}	
%		\foreach \x in {1} {
%	\addplot +[mark=none,   ] table[x index=0,y index=\x,col sep=space]{Figures/Plot_data/P10.txt};
%	}	
	\end{axis}
	\end{tikzpicture}
